Contribution of exclusive diffractive processes to the measured azimuthal asymmetries in SIDIS

Hadron leptoproduction in Semi-Inclusive measurements of Deep-Inelastic Scattering (SIDIS) on unpolarised nucleons allows one to get information on the intrinsic transverse momentum of quarks in a nucleon and on the Boer-Mulders function through the measurement of azimuthal modulations in the cross section. These modulations were recently measured by the HERMES experiment at DESY on proton and deuteron targets, and by the COMPASS experiment using the CERN SPS muon beam and a $^6$LiD target. In both cases, the amplitudes of the $\cos\phi_h$ and $\cos 2\phi_h$ modulations show strong kinematic dependences for both positive and negative hadrons. It has been known since some time that the measured final-state hadrons in those SIDIS experiments receive a contribution from exclusive diffractive production of vector mesons, particularly important at large values of $z$, the fraction of the virtual photon energy carried by the hadron. In previous measurements of azimuthal asymmetries this contribution was not taken into account, because it was not known that it could distort the azimuthal modulations. Presently, a method to evaluate the contribution of the exclusive reactions to the azimuthal asymmetries measured by COMPASS has been developed. The subtraction of this contribution results in a better understanding of the kinematic effects, and the remaining non-zero $\cos 2\phi_h$ modulation gives indication for a non-zero Boer-Mulders effect.

==> AuthorsNPB2019_oleg.tex <==
J.~Agarwala\Irefn{triest_i}\Aref{JA},
M.G.~Alexeev\Irefnn{turin_u}{turin_i},
G.D.~Alexeev\Irefn{dubna}, %1
A.~Amoroso\Irefnn{turin_u}{turin_i},
V.~Andrieux\Irefnn{cern}{illinois},
N.V.~Anfimov\Irefn{dubna}, %2
V.~Anosov\Irefn{dubna}, %3
K.~Augsten\Irefnn{dubna}{praguectu}, %2 phd
W.~Augustyniak\Irefn{warsaw},
C.D.R.~Azevedo\Irefn{aveiro},
B.~Bade{\l}ek\Irefn{warsawu},
F.~Balestra\Irefnn{turin_u}{turin_i},
M.~Ball\Irefn{bonniskp},
J.~Barth\Irefn{bonniskp},
R.~Beck\Irefn{bonniskp},
Y.~Bedfer\Irefn{saclay},
J.~Berenguer~Antequera\Irefnn{turin_u}{turin_i},
J.~Bernhard\Irefnn{mainz}{cern},
M.~Bodlak\Irefn{praguecu},
P.~Bordalo\Irefn{lisbon}\Aref{A},
F.~Bradamante\Irefn{triest_i},
A.~Bressan\Irefnn{triest_u}{triest_i},
M.~B\"uchele\Irefn{freiburg},
V.~E.~Burtsev\Irefn{tomsk},
W.-C.~Chang\Irefn{taipei},
C.~Chatterjee\Irefnn{triest_u}{triest_i},
M.~Chiosso\Irefnn{turin_u}{turin_i},
A.~G.~Chumakov\Irefn{tomsk},
S.-U.~Chung\Irefn{munichtu}\Aref{B},\Aref{B1}
A.~Cicuttin\Irefn{triest_i}\Aref{C}
P.~M.~M.~Correia\Irefn{aveiro},
M.L.~Crespo\Irefn{triest_i}\Aref{C},
D.~D'Ago\Irefnn{triest_i}{triest_u},
S.~Dalla Torre\Irefn{triest_i},
S.S.~Dasgupta\Irefn{calcutta},
S.~Dasgupta\Irefn{triest_i},
I.~Denisenko\Irefn{dubna},
O.Yu.~Denisov\Irefn{turin_i},%\CorAuth,
L.~Dhara\Irefn{calcutta},
S.V.~Donskov\Irefn{protvino},
N.~Doshita\Irefn{yamagata},
Ch.~Dreisbach\Irefn{munichtu},
W.~D\"unnweber\Arefs{D},
R.~R.~Dusaev\Irefn{tomsk},
A.~Efremov\Irefn{dubna}, %4
P.D.~Eversheim\Irefn{bonniskp},
M.~Faessler\Arefs{D},
A.~Ferrero\Irefn{saclay},
M.~Finger\Irefn{praguecu},
M.~Finger~jr.\Irefn{praguecu},
H.~Fischer\Irefn{freiburg},
C.~Franco\Irefn{lisbon},
%N.~du~Fresne~von~Hohenesche\Irefn{mainz},
J.M.~Friedrich\Irefn{munichtu},
V.~Frolov\Irefnn{dubna}{cern},   %5
%E.~Fuchey\Irefn{saclay},
F.~Gautheron\Irefnn{bochum}{illinois},
O.P.~Gavrichtchouk\Irefn{dubna}, %6
S.~Gerassimov\Irefnn{moscowlpi}{munichtu},
J.~Giarra\Irefn{mainz},
I.~Gnesi\Irefnn{turin_u}{turin_i},
M.~Gorzellik\Irefn{freiburg}\Aref{F},
A.~Grasso\Irefnn{turin_u}{turin_i},
A.~Gridin\Irefn{dubna},
M.~Grosse Perdekamp\Irefn{illinois},
B.~Grube\Irefn{munichtu},
A.~Guskov\Irefn{dubna}, %7
%D.~Hahne\Irefn{bonnpi},
%G.~Hamar\Irefnn{triest_u}{triest_i},
D.~von~Harrach\Irefn{mainz},
R.~Heitz\Irefn{illinois},
F.~Herrmann\Irefn{freiburg},
N.~Horikawa\Irefn{nagoya}\Aref{G},
N.~d'Hose\Irefn{saclay},
C.-Y.~Hsieh\Irefn{taipei}\Aref{H},
S.~Huber\Irefn{munichtu},
S.~Ishimoto\Irefn{yamagata}\Aref{I},
A.~Ivanov\Irefn{dubna},
T.~Iwata\Irefn{yamagata},
M.~Jandek\Irefn{praguectu},
V.~Jary\Irefn{praguectu},
R.~Joosten\Irefn{bonniskp},
P.~J\"org\Irefn{freiburg}\Aref{J},
E.~Kabu\ss\Irefn{mainz},
F.~Kaspar\Irefn{munichtu},
A.~Kerbisi\Irefnn{triest_u}{triest_i},
B.~Ketzer\Irefn{bonniskp},
G.V.~Khaustov\Irefn{protvino},
Yu.A.~Khokhlov\Irefn{protvino}\Aref{K},%\Aref{v},
Yu.~Kisselev\Irefn{dubna}, %9
F.~Klein\Irefn{bonnpi},
J.H.~Koivuniemi\Irefnn{bochum}{illinois},
V.N.~Kolosov\Irefn{protvino},
K.~Kondo~Horikawa\Irefn{yamagata},
I.~Konorov\Irefnn{moscowlpi}{munichtu},
V.F.~Konstantinov\Irefn{protvino},
A.M.~Kotzinian\Irefn{turin_i}\Aref{L},
O.M.~Kouznetsov\Irefn{dubna}, %10
A.~Koval\Irefn{warsaw},
Z.~Kral\Irefn{praguecu},
%M.~Kr\"amer\Irefn{munichtu},
F.~Krinner\Irefn{munichtu},
%Z.V.~Kroumchtein\Irefn{dubna}, %11
Y.~Kulinich\Irefn{illinois},
F.~Kunne\Irefn{saclay},
K.~Kurek\Irefn{warsaw},
R.P.~Kurjata\Irefn{warsawtu},
A.~Kveton\Irefn{praguecu},
K.~Lavickova\Irefn{praguecu},
S.~Levorato\Irefn{triest_i},
Y.-S.~Lian\Irefn{taipei}\Aref{M},
J.~Lichtenstadt\Irefn{telaviv},
P.-J.~Lin\Irefn{saclay}\Aref{b},
R.~Longo\Irefn{illinois},
V.~E.~Lyubovitskij\Irefn{tomsk}\Aref{N},
A.~Maggiora\Irefn{turin_i},
A.~Magnon\Irefn{retired},
N.~Makins\Irefn{illinois},
N.~Makke\Irefn{triest_i}\Aref{C},
G.K.~Mallot\Irefn{cern},
A.~Maltsev\Irefn{dubna},
S.~A.~Mamon\Irefn{tomsk},
B.~Marianski\Irefn{warsaw},
A.~Martin\Irefnn{triest_u}{triest_i},%\CorAuth,
J.~Marzec\Irefn{warsawtu},
J.~Matou{\v s}ek\Irefnn{triest_u}{triest_i},  %also {triest_u}
T.~Matsuda\Irefn{miyazaki},
G.~Mattson\Irefn{illinois},
G.V.~Meshcheryakov\Irefn{dubna}, %12
M.~Meyer\Irefnn{illinois}{saclay},
W.~Meyer\Irefn{bochum},
Yu.V.~Mikhailov\Irefn{protvino},
M.~Mikhasenko\Irefnn{bonniskp}{cern},
E.~Mitrofanov\Irefn{dubna},  %3 phd
N.~Mitrofanov\Irefn{dubna},  %4 phd
Y.~Miyachi\Irefn{yamagata},
A.~Moretti\Irefnn{triest_u}{triest_i},
A.~Nagaytsev\Irefn{dubna}, %13
C.~Naim\Irefn{saclay},
D.~Neyret\Irefn{saclay},
J.~Nov{\'y}\Irefn{praguectu},
W.-D.~Nowak\Irefn{mainz},
G.~Nukazuka\Irefn{yamagata},
A.S.~Nunes\Irefn{lisbon},
A.G.~Olshevsky\Irefn{dubna}, %14
M.~Ostrick\Irefn{mainz},
D.~Panzieri\Irefn{turin_i}\Aref{O},
B.~Parsamyan\Irefnn{turin_u}{turin_i},
S.~Paul\Irefn{munichtu},
H.~Pekeler\Irefn{bonniskp},
J.-C.~Peng\Irefn{illinois},
F.~Pereira\Irefn{aveiro},
M.~Pe{\v s}ek\Irefn{praguecu},
D.V.~Peshekhonov\Irefn{dubna}, %15
M.~Pe{\v s}kov\'a\Irefn{praguecu},
N.~Pierre\Irefnn{mainz}{saclay},
S.~Platchkov\Irefn{saclay},
J.~Pochodzalla\Irefn{mainz},
V.A.~Polyakov\Irefn{protvino},
J.~Pretz\Irefn{bonnpi}\Aref{P},
M.~Quaresma\Irefnn{taipei}{lisbon},
C.~Quintans\Irefn{lisbon},
S.~Ramos\Irefn{lisbon}\Aref{A},
%C.~Regali\Irefn{freiburg},
G.~Reicherz\Irefn{bochum},
C.~Riedl\Irefn{illinois},
T.~Rudnicki\Irefn{warsawu},
D.I.~Ryabchikov\Irefnn{protvino}{munichtu},
A.~Rybnikov\Irefn{dubna}, %6 phd
A.~Rychter\Irefn{warsawtu},
V.D.~Samoylenko\Irefn{protvino},
A.~Sandacz\Irefn{warsaw},
S.~Sarkar\Irefn{calcutta},
I.A.~Savin\Irefn{dubna}, %16
G.~Sbrizzai\Irefn{triest_i},
H.~Schmieden\Irefn{bonnpi},
A.~Selyunin\Irefn{dubna}, %7 phd
%L.~Silva\Irefn{lisbon},
L.~Sinha\Irefn{calcutta},
M.~Slunecka\Irefnn{dubna}{praguecu}, %17
J.~Smolik\Irefn{dubna}, %18
%F.~Sozzi\Irefn{triest_i},
A.~Srnka\Irefn{brno},
D.~Steffen\Irefnn{cern}{munichtu},
M.~Stolarski\Irefn{lisbon},%\CorAuth,
O.~Subrt\Irefnn{cern}{praguectu},
M.~Sulc\Irefn{liberec},
H.~Suzuki\Irefn{yamagata}\Aref{G},
A.~Szabelski\Irefnn{triest_u}{triest_i},
%T.~Szameitat\Irefn{freiburg}\Aref{F},
P.~Sznajder\Irefn{warsaw},
S.~Tessaro\Irefn{triest_i},
F.~Tessarotto\Irefn{triest_i},%\CorAuth,
A.~Thiel\Irefn{bonniskp},
J.~Tomsa\Irefn{praguecu},
F.~Tosello\Irefn{turin_i},
A.~Townsend\Irefn{illinois},
V.~Tskhay\Irefn{moscowlpi},
S.~Uhl\Irefn{munichtu},
B.~I.~Vasilishin\Irefn{tomsk},
A.~Vauth\Irefnn{bonnpi}{cern},
B.~M.~Veit\Irefnn{mainz}{cern},
J.~Veloso\Irefn{aveiro},
B.~Ventura\Irefn{saclay},
A.~Vidon\Irefn{saclay},
M.~Virius\Irefn{praguectu},
M.~Wagner\Irefn{bonniskp},
S.~Wallner\Irefn{munichtu},
M.~Wilfert\Irefn{mainz},
K.~Zaremba\Irefn{warsawtu},
P.~Zavada\Irefn{dubna}, %20
M.~Zavertyaev\Irefn{moscowlpi},
M.~Zemko\Irefn{praguecu},
E.~Zemlyanichkina\Irefn{dubna}, %21
Y.~Zhao\Irefn{triest_i} and
M.~Ziembicki\Irefn{warsawtu}
% \end{flushleft}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% institutes
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\item \Idef{bielefeld}{Universit\"at Bielefeld, Fakult\"at f\"ur Physik, 33501 Bielefeld, Germany\Arefs{l}}
%\item \Idef{munichlmu}{Ludwig-Maximilians-Universit\"at M\"unchen, Department f\"ur Physik, 80799 Munich, Germany\Arefs{l}\Arefs{r}}
\begin{Authlist}
\item \Idef{aveiro}{University of Aveiro, Dept.\ of Physics, 3810-193 Aveiro, Portugal}
\item \Idef{bochum}{Universit\"at Bochum, Institut f\"ur Experimentalphysik, 44780 Bochum, Germany\Arefs{Q},\Arefs{R}}
\item \Idef{bonniskp}{Universit\"at Bonn, Helmholtz-Institut f\"ur  Strahlen- und Kernphysik, 53115 Bonn, Germany\Arefs{Q}}
\item \Idef{bonnpi}{Universit\"at Bonn, Physikalisches Institut, 53115 Bonn, Germany\Arefs{Q}}
\item \Idef{brno}{Institute of Scientific Instruments, AS CR, 61264 Brno, Czech Republic\Arefs{S}}
\item \Idef{calcutta}{Matrivani Institute of Experimental Research \& Education, Calcutta-700 030, India\Arefs{T}}
\item \Idef{dubna}{Joint Institute for Nuclear Research, 141980 Dubna, Moscow region, Russia\Arefs{E}} 
\item \Idef{freiburg}{Universit\"at Freiburg, Physikalisches Institut, 79104 Freiburg, Germany\Arefs{Q},\Arefs{R}}
\item \Idef{cern}{CERN, 1211 Geneva 23, Switzerland}
\item \Idef{liberec}{Technical University in Liberec, 46117 Liberec, Czech Republic\Arefs{S}}
\item \Idef{lisbon}{LIP, 1649-003 Lisbon, Portugal\Arefs{U}}
\item \Idef{mainz}{Universit\"at Mainz, Institut f\"ur Kernphysik, 55099 Mainz, Germany\Arefs{Q}}
\item \Idef{miyazaki}{University of Miyazaki, Miyazaki 889-2192, Japan\Arefs{V}}
\item \Idef{moscowlpi}{Lebedev Physical Institute, 119991 Moscow, Russia}
\item \Idef{munichtu}{Technische Universit\"at M\"unchen, Physik Dept., 85748 Garching, Germany\Arefs{Q},\Arefs{D}}
\item \Idef{nagoya}{Nagoya University, 464 Nagoya, Japan\Arefs{V}}
\item \Idef{praguecu}{Charles University in Prague, Faculty of Mathematics and Physics, 18000 Prague, Czech Republic\Arefs{S}}
\item \Idef{praguectu}{Czech Technical University in Prague, 16636 Prague, Czech Republic\Arefs{S}}
\item \Idef{protvino}{State Scientific Center Institute for High Energy Physics of National Research Center `Kurchatov Institute', 142281 Protvino, Russia}
\item \Idef{saclay}{IRFU, CEA, Universit\'e Paris-Saclay, 91191 Gif-sur-Yvette, France\Arefs{R}}
\item \Idef{taipei}{Academia Sinica, Institute of Physics, Taipei 11529, Taiwan\Arefs{W}}
\item \Idef{telaviv}{Tel Aviv University, School of Physics and Astronomy, 69978 Tel Aviv, Israel\Arefs{X}}
\item \Idef{triest_u}{University of Trieste, Dept.\ of Physics, 34127 Trieste, Italy}
\item \Idef{triest_i}{Trieste Section of INFN, 34127 Trieste, Italy}
\item \Idef{turin_u}{University of Turin, Dept.\ of Physics, 10125 Turin, Italy}
\item \Idef{turin_i}{Torino Section of INFN, 10125 Turin, Italy}
\item \Idef{tomsk}{Tomsk Polytechnic University, 634050 Tomsk, Russia\Arefs{Y}}
\item \Idef{illinois}{University of Illinois at Urbana-Champaign, Dept.\ of Physics, Urbana, IL 61801-3080, USA\Arefs{Z}}
\item \Idef{warsaw}{National Centre for Nuclear Research, 02-093 Warsaw, Poland\Arefs{a} }
\item \Idef{warsawu}{University of Warsaw, Faculty of Physics, 02-093 Warsaw, Poland\Arefs{a} }
\item \Idef{warsawtu}{Warsaw University of Technology, Institute of Radioelectronics, 00-665 Warsaw, Poland\Arefs{a} }
\item \Idef{yamagata}{Yamagata University, Yamagata 992-8510, Japan\Arefs{V} }
\item \Idef{retired}{Retired}
\end{Authlist}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% Notes
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\vspace*{-\baselineskip}
\renewcommand\theenumi{\alph{enumi}}
\begin{Authlist}
\item [{\makebox[2mm][l]{\textsuperscript{\#}}}] Corresponding authors
%%%\item [{\makebox[2mm][l]{\textsuperscript{\#}}}] Corresponding authors
%\item [{\makebox[2mm][l]{\textsuperscript{*}}}] Deceased
\item \Adef{JA}{Present address: University of Pavia, 27100 Pavia, Italy}
\item \Adef{A}{Also at Instituto Superior T\'ecnico, Universidade de Lisboa, Lisbon, Portugal}
\item \Adef{B}{Also at Dept.\ of Physics, Pusan National University, Busan 609-735, Republic of Korea}
\item \Adef{B1}{Also at at Physics Dept., Brookhaven National Laboratory, Upton, NY 11973, USA}
\item \Adef{C}{Also at Abdus Salam ICTP, 34151 Trieste, Italy}
\item \Adef{D}{Supported by the DFG cluster of excellence `Origin and Structure of the Universe' (www.universe-cluster.de) (Germany)}
\item \Adef{E}{Supported by CERN-RFBR Grant 12-02-91500}
\item \Adef{F}{Supported by the DFG Research Training Group Programmes 1102 and 2044 (Germany)}
\item \Adef{G}{Also at Chubu University, Kasugai, Aichi 487-8501, Japan\Arefs{V}}
\item \Adef{H}{Also at Dept.\ of Physics, National Central University, 300 Jhongda Road, Jhongli 32001, Taiwan}
\item \Adef{I}{Also at KEK, 1-1 Oho, Tsukuba, Ibaraki 305-0801, Japan}
\item \Adef{J}{Present address: Universit\"at Bonn, Physikalisches Institut, 53115 Bonn, Germany}
\item \Adef{K}{Also at Moscow Institute of Physics and Technology, Moscow Region, 141700, Russia}
\item \Adef{L}{Also at Yerevan Physics Institute, Alikhanian Br. Street, Yerevan, Armenia, 0036}
\item \Adef{M}{Also at Dept.\ of Physics, National Kaohsiung Normal University, Kaohsiung County 824, Taiwan}
\item \Adef{N}{Also at Institut f\"ur Theoretische Physik, Universit\"at T\"ubingen, 72076 T\"ubingen, Germany}
\item \Adef{O}{Also at University of Eastern Piedmont, 15100 Alessandria, Italy}
\item \Adef{P}{Present address: RWTH Aachen University, III.\ Physikalisches Institut, 52056 Aachen, Germany}
\item \Adef{Q}{Supported by BMBF - Bundesministerium f\"ur Bildung und Forschung (Germany)}
\item \Adef{R}{Supported by FP7, HadronPhysics3, Grant 283286 (European Union)}
\item \Adef{S}{Supported by MEYS, Grant LM20150581 (Czech Republic)}
\item \Adef{T}{Supported by B.Sen fund (India)}
\item \Adef{U}{Supported by FCT, Grants CERN/FIS-PAR/0007/2017 and  CERN/FIS-PAR/0022/2019 (Portugal)}
\item \Adef{V}{Supported by MEXT and JSPS, Grants 18002006, 20540299, 18540281 and 26247032, the Daiko and Yamada Foundations (Japan)}
\item \Adef{W}{Supported by the Ministry of Science and Technology (Taiwan)}
\item \Adef{X}{Supported by the Israel Academy of Sciences and Humanities (Israel)}
\item \Adef{Y}{Supported by the Russian Federation  program ``Nauka'' (Contract No. 0.1764.GZB.2017) (Russia)}
\item \Adef{Z}{Supported by the National Science Foundation, Grant no. PHY-1506416 (USA)}
\item \Adef{a}{Supported by NCN, Grant 2017/26/M/ST2/00498 (Poland)}
\item \Adef{b}{Supported by ARN,  France with the P2IO LabEx (ANR-10-LBX-0038) in the framework ``Investissements d'Avenir'' (ANR-11-IDeX-003-01)}
\end{Authlist}

